DREQ: Document Re-Ranking Using Entity-based Query Understanding

While entity-oriented neural IR models have advanced significantly, they often overlook a key nuance: the varying degrees of influence individual entities within a document have on its overall relevance. Addressing this gap, we present DREQ, an entity-oriented dense document re-ranking model. Uniquely, we emphasize the query-relevant entities within a document's representation while simultaneously attenuating the less relevant ones, thus obtaining a query-specific entity-centric document representation. We then combine this entity-centric document representation with the text-centric representation of the document to obtain a "hybrid" representation of the document. We learn a relevance score for the document using this hybrid representation. Using four large-scale benchmarks, we show that DREQ outperforms state-of-the-art neural and non-neural re-ranking methods, highlighting the effectiveness of our entity-oriented representation approach.

==> tex-files/figures/cluster-rq4.tex <==
% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.4\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/dbi.pdf} 
%         \caption{Caption for chart 1.}
%         \label{fig:chart1}
%     \end{minipage}\hfill 
%     \begin{minipage}{0.4\textwidth}
%         \centering
%         \includegraphics[width=0.9\linewidth]{images/ndcg.pdf}
%         \caption{Caption for chart 2.}
%         \label{fig:chart2}
%     \end{minipage}

% \end{figure}

\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{images/dbi.pdf} 
        \caption{DB Score vs top-$k$ entities.}
        \label{fig:rq4-dbi}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{images/ndcg.pdf}
        \caption{nDCG@20 vs top-$k$ entities.}
        \label{fig:rq4-ndcg}
    \end{subfigure}
    \caption{Variation in ranking quality as the number of query expansion entities increases on Robust04 title queries. We observe that the DBS values consistently increase with the increase in K (left). This indicates that as more entities are added, the cluster compactness decreases, and/or the separation between the clusters decreases. This explains the invariant performance of \texttt{DREQ} across different top-K entities (right): the added entities do not contribute significantly new or distinct information to the queries. Hence, performance of \texttt{DREQ} is robust.}
    \label{fig:rq4-dbi-and-ndcg}
\end{figure}

==> tex-files/figures/difficulty_test.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=0.4]{images/difficulty_test.pdf}
    \caption{Difficulty test for nDCG@20 on TREC Robust04 title queries, comparing different re-ranking systems. Candidate ranking: BM25+RM3. 5\% most difficult queries for BM25+RM3 to the left and the 5\% easiest ones to the right. Performance reported as macro-averages across queries.  For the most difficult queries
    (0-25\%), relevant documents are promoted to the top of the ranking using \texttt{DREQ}.}
    \label{fig:diff-test}
\end{figure}

==> tex-files/figures/embedding_plots.tex <==


\begin{figure}[t]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{images/plot_fold_0_dreq_only_text_emb.pdf} 
        \caption{No document entity embedding.}
        \label{fig:plot-emb-only-text}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        \includegraphics[width=1\linewidth]{images/plot_fold_0_dreq_full.pdf}
        \caption{With document entity embeddings.}
        \label{fig:plot-emb-full}
    \end{subfigure}
    \caption{Visualizing clusters of relevant documents using t-SNE. We observe better clusters of relevant documents using document entity embeddings (right).}
    \label{fig:plot-emb}
\end{figure}

==> tex-files/sections/introduction.tex <==
\section{Introduction}
\label{sec:Introduction}

%Information retrieval has seen monumental progress with the advent of deep neural models, particularly the likes of BERT \cite{devlin2018bert}. 
Central to the success of neural IR models is often the ``retrieve-then-rerank'' paradigm where some candidate documents retrieved using an efficient retrieval method (e.g., BM25 \cite{robertson2009probabilistic}) are re-ranked using more computationally-heavy scoring functions.
%Initially, a set of candidate documents is retrieved using an efficient retrieval method (e.g., BM25 \cite{robertson2009probabilistic}). These candidate documents are then re-ranked using more computationally-heavy scoring functions such as BERT-based cross-encoders \cite{reimers2019sentence,devlin2018bert}. 
The efficacy of BERT \cite{devlin2018bert} in this framework has been aptly demonstrated earlier \cite{nogueira2019passage,nogueira2019multi}, with subsequent research \cite{liu2019roberta,he2020deberta,clark2020electra} enhancing the effectiveness further.
%with substantial performance gains on prominent benchmarks. Moreover, subsequent research \cite{liu2019roberta,he2020deberta,clark2020electra} has fine-tuned the model pretraining, thereby enhancing the efficiency and potency of the ranking process.
%
Yet, amid these advancements, the role of entities in neural-IR remains under-explored. Entities carry a wealth of semantic information (e.g., types and relations) and act as explicit textual anchors, bridging unstructured text and structured knowledge. Previous work \cite{ensan2017document,xiong2015esdrank,xiong2017word,liu2015latent,raviv2016document} shows their importance in feature-based retrieval systems; however, contemporary neural-IR models have barely begun to integrate them effectively. The intersection of knowledge graph semantics, inherent in entity-oriented search, with the dense vector representations characteristic of neural-IR models represents a promising research avenue.
%Recent work \cite{tran2022dense} has underscored the untapped potential of entities in neural-IR.
%Works by Liu et al. \cite{liu-etal-2018-entity} in 2018, and more recently, by Tran and Yates \cite{tran2022dense} in 2022 have highlighted the potential of entities in neural-IR. 
%While entity-oriented search taps into human knowledge via knowledge graph semantics, neural-IR capitalizes on vector representations learnt from large datasets. The synergy between these two powerful methodologies remains an intriguing, yet largely unexplored territory. 

%Moreover, while recent research \cite{kulkarni2023ladr,macavaney2022adaptive} has focused on enhancing the recall of the initial candidate set of documents used in the retrieve-then-rerank paradigm, the overarching goal in IR has always been to achieve a balance between recall and precision, specifically  precision at top ranks as measured by metrics like nDCG@10 and MAP.









% The domain of information retrieval has witnessed substantial advancements with the introduction of deep neural models, most notably, architectures like BERT \cite{devlin2018bert}. 
% %Designed to comprehend intricate textual patterns, these models have remarkably elevated document retrieval precision. 
% The pinnacle of their effectiveness is often achieved in a two-tiered paradigm: retrieve-then-rerank. Initially, an efficient retrieval strategy (e.g., BM25 \cite{robertson2009probabilistic}) curates a preliminary pool of candidate documents. These are subsequently re-ranked using sophisticated, computationally-intensive scoring functions, like BERT-based cross-encoders. Pioneering efforts by Nogueira et al. \cite{nogueira2019passage,nogueira2019multi}, have showcased the power of BERT in the retrieve-then-rerank paradigm, resulting in significant performance enhancements on benchmarks like the MS MARCO passage ranking test collection. Further advancements \cite{liu2019roberta,he2020deberta,clark2020electra} have refined the model pretraining, accelerating the ranking process and enhancing efficacy. 

% Despite these advancements, a pivotal aspect that warrants exploration in the context of neural-IR is the role of semantic understanding in document ranking. Entities, which are discrete units with rich semantic information, offer a promising avenue in this regard. Entities serve as explicit anchors in text, representing specific people, places, concepts, or events. The rich semantic information associated with entities (e.g., types and relations to other entities) allows for a deeper and more structured understanding of textual content, bridging the gap between unstructured text and structured knowledge. While entities have historically proven their merit in document retrieval \cite{dalton2014entity,ensan2017document,xiong2015esdrank,xiong2017word,liu2015latent,raviv2016document}, recent neural-IR models have scarcely tapped into their potential. Notable efforts by Liu et al. \cite{liu-etal-2018-entity} in 2018, and more recently, by Tran and Yates \cite{tran2022dense} in 2022, have emphasized the advantages of incorporating entities in document ranking. Yet, there is a notable gap in current research when it comes to merging entity-based knowledge with advanced neural IR methodologies.

% Entity-oriented search and neural-IR, in essence, are pushing the boundaries of search from two distinct directions. The former harnesses human knowledge encapsulated within entities and the semantics of knowledge graphs, demonstrating significant promise in feature-based ranking systems. Contrarily, neural-IR capitalizes on distributed representations and neural network intricacies, deriving sophisticated ranking models from vast training datasets. The interplay between these two methodologies remains largely uncharted, raising the question of whether the proven benefits of entity-oriented search in feature-based systems extend equivalently to neural-IR mechanisms.

Against this backdrop, in this work\footnote{\textbf{Code and data to be released upon acceptance.}}, we introduce \textit{\textbf{D}ocument \textbf{R}e-ranking using \textbf{E}ntity-based \textbf{Q}uery Understanding} (\texttt{DREQ}), an entity-oriented neural re-ranking model that extends the conventional ``retrieve-then-rerank'' paradigm by introducing an innovative intermediate step. We aptly term our methodology ``retrieve-harness-rerank'' %\footnote{This term was recently coined at the tutorial on ``Neuro-Symbolic Representations for IR'' held at ECIR 2023 and SIGIR 2024.},
emphasizing our process of initially retrieving a candidate set of documents, then harnessing the rich information from entities present in this set, followed by a refined re-ranking of the candidates. %While recent work \cite{kulkarni2023ladr,macavaney2022adaptive} has focused on enhancing the recall of this candidate set, 
%We focus on enhancing the precision at top ranks as measured by metrics such nDCG@10 and MAP.
%the overarching goal in IR has always been to achieve a balance between recall and precision, specifically  precision at top ranks as measured by metrics such nDCG@10 and MAP. 
%as \textit{Normalized Discounted Cumulative Gain} and \textit{Mean Average Precision} at certain cut-off ranks. 
%Consequently, at the core of our methodology is the utilization of knowledge about entities in candidate documents to enhance precision at top ranks. 
Our approach integrates entity-centric and text-centric representations of documents. At the heart of our approach is the intuition that entities within a document act as pivotal indicators of the document's thematic breadth, offering crucial insights into the document's relevance to a query. Nonetheless, the significance of these entities is contingent upon their relevance to the query. Hence, we pool the entities from all candidate documents and rank them based on their relevance to the given query. We cross-reference entities in each candidate document with entities from this ranked list, aggregating the embeddings of matched entities into a unified representation, where entity embeddings are weighted by their relevance scores.
%This aggregation isn't arbitrary: Entity embeddings are weighted by their relevance scores. 
Consequently, our model prioritizes more important (relevant) entities, resulting in a nuanced, \textit{query-tuned entity-centric document representation}.
%Consequently, while our model accommodates a breadth of entities, it bestows more importance on those of higher relevance, resulting in a nuanced, query-tuned entity-centric representation of the document. 
\input{tex-files/figures/example-intro}

%Our methodology isn't solely reliant on entities. 
Furthermore, recognizing that the raw text of a document captures the document's overarching semantic context, we also derive a broader text-centric representation of the document, complementing the focused entity-centric perspective. We meld the entity-centric and text-centric representations of the document, resulting in a ``hybrid'' document representation. This hybrid representation imbibes insights about what the query specifically seeks. This fusion allows \texttt{DREQ} to extract nuanced relevance signals for a deeper understanding of relevance.
%This intricate melding enables \texttt{DREQ} to derive nuanced relevance signals to offer a refined understanding of relevance.




%entities within documents can serve as indicators of the key concepts the query aims to address. Identifying the key query-relevant entities in candidate documents could provide a clearer perspective on the relevance of these documents to the given query. To operationalize this, we pool the entities from all candidate documents and subsequently rank them based on their relevance to the given query. We leverage this entity ranking to learn \textit{query-specific} and \textit{entity-centric} representations of the candidate documents. 
%At the heart of our approach is the intuition that entities can act as surrogate markers for the most vital concepts underpinning the query's meaning. If we know which entities from the candidate documents are most important for understanding the query, then we can use these entities to guide the model to the most relevant documents. To opertionzalize this, we first rank the entities in the candidate documents using BERT. Using this entity ranking, we derive a query-specific entity-centric document representation. 
%Based on the intuition that not all entities in a document contribute equally to its relevance for a particular query, we weigh the embeddings of entities in a candidate document based on scores of these entities in the entity ranking. These entity scores serve as ``attention'' weights, emphasizing entities that are more pertinent to the query. 
%Complementing this focused entity-centric perspective, we also derive a broader text-centric representation of the document, capturing the document's overarching semantic context. 
%a method grounded in previous work \cite{nogueira2019passage,zhuang2023rankt5}. 
%Simultaneously, we also apply a similar dual representation learning process to the query, using the top-$k$ entities from the entity ranking to enrich the query's representation. We meld the entity-centric and text-centric representations for both the query and document, resulting in ``hybrid'' query and document representations. %infused with both contextual depth and precise relevance details.
%We use the top-$k$ entities from the entity ranking, acting as indicators of broad concepts crucial for understanding the query, to enrich the query's representation. This entity-centric representation is combined with the query's textual representation to obtain a comprehensive understanding of the query. 
%The document's query-specific hybrid representation imbibes insights about what the query specifically seeks, while the query's hybrid representation defines what genuine relevance means for that particular query. This intricate melding enables \texttt{DREQ} to derive nuanced relevance signals to offer a refined understanding of relevance. %Experimental evaluation on four large-scale document ranking benchmarks using five diverse query sets demonstrates the effectiveness of \texttt{DREQ} to promote relevant documents to the top while demoting the non-relevant documents, thereby increasing the precision at the top ranks.

\textit{\textbf{Contributions.}} \textbf{(1)} We introduce \texttt{DREQ}, an \textit{entity-oriented re-ranking framework} that \textit{enriches the document representation} with \textit{query-specific} entity knowledge for nuanced relevance matching. \textbf{(2)} We introduce a hybrid representation learning mechanism, blending entity-centric and text-centric representations. This hybrid representation captures a document's broad context and query-specific relevance,  enhancing the precision of re-ranking. \textbf{(3)} We demonstrate that \texttt{DREQ} achieves new state-of-the-art results on four major document ranking test collections. Our analysis shows that entities play a crucial role in this.% performance improvement.

% \begin{enumerate}[leftmargin=*]
%     \item  We introduce \texttt{DREQ}, an entity-oriented re-ranking framework that enriches query and document representations with external entity knowledge for nuanced relevance matching.
    
%     %We propose \texttt{DREQ}, a novel entity-oriented dense document re-ranking framework. Our approach leverages external knowledge about entities in candidate documents to learn an enriched query and document representation that allows the model to learn more nuanced relevance matching signals.

%     \item We introduce a hybrid representation mechanism that combines entity-centric and text-centric representations. For documents, this hybrid representation captures both the broad semantic context and the nuanced, query-specific relevance details. For the query, it captures what it means to be relevant for that query, thereby providing a holistic view that enhances the precision of the re-ranking process. 

%     \item We demonstrate that \texttt{DREQ}, employing our ``retrieve-harness-rerank'' paradigm, achieves new state-of-the-art results on four major document ranking test collections across five varied query sets. Our analysis shows that entities play a crucial role in this performance improvement.

%     %\item We demonstrate that entities allow \texttt{DREQ} to promote relevant documents to the top while demoting non-relevant documents, thereby increasing precision at the top ranks. 
% \end{enumerate}




==> tex-files/sections/related-work-new.tex <==
\section{Related Work}
\label{sec:Related Work}

\subsection{Entity-Oriented Search}
\label{subsec:Entity-Oriented Search}

Early attempts at entity-oriented search utilized entities primarily for query expansion. A key development in this domain was made by Meij et al. \cite{meij2010conceptual} who proposed a double translation process. The method first translated a query into relevant entities and then employed the terms associated with these entities for query expansion. Dalton et al. \cite{dalton2014entity} later improved upon this approach with Entity Query Feature Expansion (EQFE), which enriched document retrieval by expanding query context using entity-related features.

However, the field soon recognized the integral role of entities in search applications, leading to a shift in approach. Instead of merely using entities for query expansion, researchers started treating them as a latent layer while preserving the original document/query representations intact \cite{gabrilovich2009wikipedia,liu2015latent}. This resulted in innovative methods that projected queries and documents into a high-dimensional latent entity space. Each dimension in this space corresponded to a unique entity, thereby uncovering hidden semantic relationships between queries and documents and enhancing the retrieval of relevant content. Notable works in this regard include the Explicit Semantic Analysis \cite{gabrilovich2009wikipedia} method, which generated a vector-based representation of semantics using ``concept vectors'' from knowledge repositories like Wikipedia. On the other hand, the Latent Entity Space model \cite{liu2015latent} leveraged entities to determine the relevance between documents and queries based on their respective positions along each entity-informed dimension. Similarly, EsdRank \cite{xiong2015esdrank} utilized semi-structured data such as controlled vocabularies and knowledge bases to create connectors between queries and documents, thereby pioneering a new approach to document representation and ranking based on interrelated entities.

The success of this trajectory of research inspired a significant shift towards methodologies that consider entities within documents not as a latent layer, but rather as explicit, integral elements of the retrieval model. In such models, entities are seen as fundamental constituents that coexist harmoniously with the traditional term-based representations. One such innovative approach is the creation of entity-based language models. Raviv et al. \cite{raviv2016document} focused on the influence of explicit entity markup within queries and documents, balancing between term-based and entity-based information for document ranking. Ensan et al. \cite{ensan2017document} take a semantically-driven path, creating the Semantic Enabled Language Model which ranks documents based on the semantic relatedness to the query. 

Another influential line of work primarily spearheaded by Xiong et al. presents entities in a distinct ``bag-of-entities'' representation alongside the conventional ``bag-of-terms''. This dual-layered approach enhances the document retrieval process by encapsulating the semantics of both term and entity-based methodologies. For instance, Explicit Semantic Ranking \cite{xiong2017explicit} utilized a knowledge graph for creating ``soft matches'' in the entity space, while the the Word-Entity Duet Model \cite{xiong2017word} captured multiple interactions between queries and documents using a mixture of term and entity-based vectors. Recognizing the potential pitfalls of incorrect entity linking, they further developed the AttR-Duet \cite{xiong2017word} model, implementing an attention mechanism to downplay noisy query entities. Following this, the Kernel Entity Salience Model \cite{xiong2018towards}, estimates an entity's prominence within a document by modeling interactions between entities and words, creating a comprehensive model for enhanced document retrieval. 

%This evolution in document retrieval research has demonstrated the significant potential of integrating entities explicitly within retrieval models, opening new avenues for enhancing document retrieval effectiveness.

% \subsection{Neural IR}
% \label{subsec:Neural IR}

\textbf{Neural IR.} Recently, deep learning has transformed text ranking, removing the need for handcrafted features and fostering semantic matching. Before BERT \cite{devlin2018bert}, models either created vector representations \cite{huang2013learning,shen2015entity,mitra2019an,nalisnick2016improving} for queries and documents  or built similarity matrices to capture term interactions \cite{guo2016drmm,xiong2017end,hui-etal-2017-pacrr,hui2018copacrr,dai2018cknrm}. The advent of BERT  and its derivatives \cite{liu2019roberta,clark2020electra,he2020deberta,zhang-etal-2019-ernie,jiang2020convbert} in a retrieve-then-rerank \cite{nogueira2019passage,nogueira2019multi} framework ushered in models like Birch \cite{akkalyoncu-yilmaz-etal-2019-cross} and BERT-MaxP \cite{dai2019deeper}, emphasizing sentence or passage relevance. Subsequent models, such as CEDR \cite{macavaney2019ceder} and PARADE \cite{li2020parade}, utilized BERT's contextual embeddings, with the latter aggregating passage representations. Concurrently, ERNIE \cite{zhang-etal-2019-ernie} enhanced BERT with knowledge graphs and vast text corpora.
%, there was also a push to move away from BERT. Notably, Hofstatter et al. \cite{hofstatter2019tu,hofstatter2020interpretable}  employed distinct transformer stacks for learning query and document term representations.

%Deep learning has revolutionized text ranking by eliminating the need for handcrafted features and enabling semantic matching methods. Pre-BERT era saw the rise of representation-based models \cite{huang2013learning,shen2015entity,mitra2019an,nalisnick2016improving}, which focus on creating vector representations of queries and documents, and interaction-based models \cite{guo2016drmm,xiong2017end,hui-etal-2017-pacrr,hui2018copacrr,dai2018cknrm}, which build a similarity matrix to capture term interactions in a query and a document. The introduction of BERT \cite{devlin2018bert} and its variants \cite{liu2019roberta,clark2020electra,he2020deberta,zhang-etal-2019-ernie,jiang2020convbert}, used in a retrieve-then-rerank \cite{nogueira2019passage,nogueira2019multi} framework, opened a new chapter in text ranking, bringing about models like Birch \cite{akkalyoncu-yilmaz-etal-2019-cross}  and BERT-MaxP \cite{dai2019deeper}, which estimate the relevance of individual sentences or passages. Models such as CEDR \cite{macavaney2019ceder} and PARADE \cite{li2020parade} went a step further by leveraging BERT's contextual embeddings, with the latter aggregating passage representations rather than individual passage scores. Simultaneously, some efforts have also focused on enriching BERT with knowledge. For example ERNIE \cite{zhang-etal-2019-ernie} uses KG embeddings and large-scale text corpora to enhance BERT.%and E-BERT ~\cite{poerner-et-al-2020-ebert}.
%
%There have also been efforts to design new neural architectures; a notable example is the Transformer Kernel \cite{hofstatter2019tu,hofstatter2020interpretable} model which separately uses transformer stacks for learning query and document term representations. %later enhanced with local self-attention \cite{hofstatter2020local} 

Meanwhile, bi-encoders emerged as a foundational mechanism in text ranking, employing distinct encoders to derive query and document vectors. For example, DPR \cite{karpukhin-etal-2020-dense} employs BERT's \texttt{[CLS]} token for both, gauging similarity through their inner product. The choice of negative examples is crucial: DPR favors BM25-retrieved passages while ANCE \cite{xiong2020ance} leans on ANN techniques. Addressing bi-encoders' challenges with term-level interactions, research has delved into multi-vector text representation, exemplified by ColBERT's \cite{khattab2020colbert} ``late interaction'' using token-level embeddings. %Another avenue is distilling complex cross-encoders to bi-encoders, exemplified by TCT-ColBERT \cite{lin2020distilling} using ColBERT for on-the-fly soft-labeling during distillation.

%Meanwhile, bi-encoders emerged as a foundational mechanism in text ranking, employing distinct encoders to derive query and document vectors. DPR \cite{karpukhin-etal-2020-dense}, for instance, leverages the \texttt{[CLS]} token from BERT to embed both the query and document, determining similarity via the inner product of these embeddings. Central to the success of bi-encoder training is the apt selection of negative examples; while DPR suggests utilizing passages retrieved by BM25, ANCE \cite{xiong2020ance} proposes to use ANN techniques for this purpose. Bi-encoders sometimes struggle with capturing detailed term-level interactions, prompting some researchers to explore text representation using multiple vectors, as seen with the ``late interaction'' using token-level embeddings from ColBERT \cite{khattab2020colbert}. Conversely, another research approach is distilling advanced cross-encoders into simpler bi-encoders, with TCT-ColBERT \cite{lin2020distilling} being a notable example, leveraging ColBERT for real-time soft-label computations during knowledge distillation.

%Despite their effectiveness, bi-encoders often grapple with capturing intricate term-level interactions. One line of research aims to address this issue by representing text using multiple vectors instead of a single vector. For example, ColBERT \cite{khattab2020colbert} generates embeddings for each token, introducing the concept of ``late interactions'' to allow intricate interplay between individual query and document terms. On the other hand, another line of research is focused on distilling ``more powerful'' cross-encoders into ``less powerful'' bi-encoders. For example, TCT-ColBERT \cite{lin2020distilling} utilizes ColBERT for on-the-fly computation of soft-labels for in-batch negatives during knowledge distillation. 

%The advent of pre-trained sequence-to-sequence models like T5 \cite{raffel2019exploring}, have surpassed the capabilities of earlier models like BERT. Innovations like MonoT5 \cite{nogueira2019document}, which assesses document relevance via probability assignment to ``true'' labels during decoding, and RankT5 \cite{zhuang2023rankt5}, which provides direct ranking scores for query-document pairs, have further pushed the boundaries in this field.

The evolution of pre-trained sequence-to-sequence models like T5 \cite{raffel2019exploring} has led to models such as MonoT5 \cite{nogueira2019document} and RankT5 \cite{zhuang2023rankt5}: The former assesses document relevance via probability assignment to ``true'' labels during decoding whereas the latter provides direct ranking scores for query-document pairs.







%Deep learning has revolutionized text ranking by enabling more flexible and semantic matching methods, and by eliminating the need for handcrafted features. The pre-BERT era was marked by two key methodologies in neural ranking: representation-based and interaction-based models. Representation-based models \cite{huang2013learning,shen2015entity,mitra2019an,nalisnick2016improving}, which focus on creating vector representations of queries and documents, measure relevance using metrics like cosine similarity. On the other hand, interaction-based models \cite{guo2016drmm,xiong2017end,hui-etal-2017-pacrr,hui2018copacrr,dai2018cknrm} build a similarity matrix that captures the interactions between terms in a query and a document. 

%The introduction of BERT \cite{devlin2018bert} significantly transformed the field of text ranking. Nogueira et al. \cite{nogueira2019passage,nogueira2019multi} spearheaded the use of BERT in a retrieve-then-rerank framework, using both pointwise and pairwise ranking models. However, BERT's fixed sequence length limit posed a challenge for ranking longer documents, prompting the creation of models such as Birch \cite{akkalyoncu-yilmaz-etal-2019-cross} and BERT-MaxP \cite{dai2019deeper}, which estimate the relevance of individual sentences or passages. Furthermore, the usefulness of BERT's contextual embeddings in neural ranking models was explored by CEDR \cite{macavaney2019ceder}, leading to the development of PARADE \cite{li2020parade}, which aggregates passage representations rather than individual passage scores.

%Bi-encoders (e.g., DPR \cite{karpukhin-etal-2020-dense}) have become a foundational tool in text representation and ranking, with the common design utilizing separate encoders to create query and document vectors, which are then compared via a simple operation such as inner product. However, 
%The Dense Passage Retriever  \cite{karpukhin-etal-2020-dense} model exemplifies this approach by using BERT's \texttt{[CLS]} token to create embeddings of queries and documents, with their similarity computed via the inner product of these embeddings. Additionally, the selection of negative examples for training has sparked discussion, with strategies ranging from mixing BM25-retrieved passages  \cite{karpukhin-etal-2020-dense} to employing Approximate Nearest Neighbor techniques, as proposed in the ANCE \cite{xiong2020ance} model.
%bi-encoders face challenges in capturing term-level interactions due to their independent encoding mechanism. To address this, ColBERT \cite{khattab2020colbert} generates dense vector representations for each token, introducing the concept of ``late interactions'' to allow intricate interplay between individual query and text terms.

%Two innovative solutions to this problem are the Poly-encoder \cite{Humeau2020Poly-encoders:} and ColBERT \cite{khattab2020colbert} models. The Poly-encoder model generates multiple context-dependent representations of a document and combines them with the query using an attention mechanism. On the other hand, the ColBERT model takes a different approach, generating dense vector representations for each token and introducing the concept of ``late interactions'' to allow intricate interplay between individual query and text terms.

%To achieve more efficiency and effectiveness, research has focused on designing new neural architectures instead of depending on overly complex models like BERT; a notable example is Transformer Kernel \cite{hofstatter2019tu,hofstatter2020interpretable} model which separately uses transformer stacks for learning query and document term representations, later enhanced with local self-attention \cite{hofstatter2020local} 

%In the quest for more efficient and effective models, prior work has also focused on redesigning neural architectures from scratch instead of relying on over-parameterized models like BERT. One exemplary stride in this direction is Hofstatter et al.'s \cite{hofstatter2019tu,hofstatter2020interpretable} Transformer Kernel model, which uses separate transformer stacks for learning contextual representations of query and document terms, later enhanced with local self-attention \cite{hofstatter2020local} 

%in their subsequent TK with Local Attention \cite{hofstatter2020local} model. 
%Adding to these innovations, Mitra et al.'s \cite{mitra2020conformer} Conformer Kernel model incorporated explicit term-matching and ``conformer'' layers, marking another leap forward in the design of optimized models for document ranking tasks.

%The advent of pre-trained sequence-to-sequence models like T5 \cite{raffel2019exploring}, have surpassed the capabilities of earlier models like BERT, enabling them to handle diverse NLP tasks. Innovations like MonoT5 \cite{nogueira2019document}, which assesses document relevance via probability assignment to ``true'' labels during decoding, and RankT5 \cite{zhuang2023rankt5}, which provides direct ranking scores for query-document pairs by fine-tuning the T5 model with pairwise or listwise ranking losses, have further pushed the boundaries in this field.

%The rise of pre-trained sequence-to-sequence models like T5 \cite{raffel2019exploring}, UniLM \cite{dong2019unified}, and BART  \cite{lewis2019bart} has broadened their use across diverse NLP tasks, exceeding the capabilities of earlier encoder-only models like BERT, which were limited to tasks not producing a sequence of tokens. Leveraging this, MonoT5 \cite{nogueira2019document} evaluates a document's relevance by assigning a probability to the ``true'' label during initial decoding. The recent introduction of RankT5 \cite{zhuang2023rankt5} has further advanced this field, offering direct ranking scores for query-document pairs by fine-tuning the T5 model with pairwise or listwise ranking losses


%While tasks not resulting in a sequence of tokens were previously managed using encoder-only models like BERT, the advent of pre-trained sequence-to-sequence models such as T5 \cite{raffel2019exploring}, UniLM \cite{dong2019unified}, and BART  \cite{lewis2019bart} has spurred their application to a wider variety of NLP tasks. Building on this, Nogueira et al. \cite{nogueira2019document} proposed MonoT5, a model fine-tuned to estimate a document's relevance by assigning a probability to the ``true'' label during the initial decoding phase. The recent introduction of RankT5 \cite{zhuang2023rankt5} has further advanced this field, offering direct ranking scores for query-document pairs by fine-tuning the T5 model with pairwise or listwise ranking losses, significantly improving ranking performance and showcasing robust zero-shot ranking capabilities on out-of-domain data.






% The emergence of deep learning introduced significant changes to text ranking, namely the liberation from exact term matching and the removal of the necessity for manual feature crafting. This evolution can be split into two primary ``eras'': the era before BERT models and the era dominated by BERT-based models. In this section, we provide a succinct overview of these eras. %However, a detailed exploration of this evolution isn't possible due to limited space, and readers are advised to refer to existing literature for a more comprehensive understanding \cite{Onal2018,mitra2018introduction,lin2020pretrained}.

% \textbf{Pre-BERT Models.} The pre-BERT era was marked by two key methodologies in neural ranking: representation-based and interaction-based models. Representation-based models \cite{huang2013learning,shen2015entity,mitra2019an,nalisnick2016improving}, which focus on creating vector representations of queries and documents, measure relevance using metrics like cosine similarity. On the other hand, interaction-based models \cite{guo2016drmm,xiong2017end,hui-etal-2017-pacrr,hui2018copacrr,dai2018cknrm} build a similarity matrix that captures the interactions between terms in a query and a document. While representation-based models are usually quicker due to the use of pre-computed document vectors, interaction-based models often demonstrate better effectiveness and the ability to capture exact match signals.

% \textbf{BERT-based Models.} The introduction of BERT \cite{devlin2018bert} significantly transformed the field of text ranking. 
% %Its application to the MS MARCO passage ranking test collection resulted in a remarkable 30\% gain in effectiveness, sparking excitement in both academia and industry.  In this regard, 
% Nogueira et al. \cite{nogueira2019passage,nogueira2019multi} pioneered the developement of a retrieve-then-rerank framework using BERT, employing both pointwise and pairwise learning-to-rank models. However, BERT's fixed sequence length of 512 tokens hindered ranking longer documents. Solutions such as Birch \cite{akkalyoncu-yilmaz-etal-2019-cross} and BERT-MaxP \cite{dai2019deeper} emerged to bypass this limitation by estimating the relevance of individual sentences or passages. CEDER \cite{macavaney2019ceder} explored whether contextual embeddings from BERT are useful when used in a neural ranking model. PARADE built on CEDER and proposed to aggregates the representations of passages from a document rather than aggregating the scores of individual passages (as done by Birch and BERT–MaxP). 

% %Some researchers have directly trained Transformers for document ranking tasks. Hofstatter et al.'s Transformer Kernel \cite{hofstatter2019tu,hofstatter2020interpretable} (TK) model learns contextual representations of query and document terms using separate transformer stacks. They further developed the TK model into the TK with local attention model (TKL) \cite{hofstatter2020local} that incorporates local self-attention. Mitra et al. \cite{mitra2020conformer} then expanded on TK, introducing the Conformer Kernel (CK) model that includes an explicit term-matching component and 'conformer' layers.

% \textbf{Bi-Encoder Models.} The concept of bi-encoders has become fundamental in the area of text representation and ranking. In a basic bi-encoder design, encoders produce query and document vectors, which are then compared via a simple operation such as inner product.  Among these, the Dense Passage Retriever \cite{karpukhin-etal-2020-dense} embeds the query and document through the \texttt{[CLS]} token from BERT, with the similarity calculated through the inner product of the embeddings. A crucial factor in DPR's training is the selection of negative examples. While some propose a mix of BM25-retrieved passages and passages from the same batch as the best strategy, Xiong et al. \cite{xiong2020ance} suggest using Approximate Nearest Neighbor techniques to identify negative examples in their ANCE model.

% \textbf{Multiple Text Representation Models.} Bi-encoders struggle to capture term-level interactions between a query and a document due to their independent encoding. Poly-encoder and ColBERT models are innovative approaches to address this limitation. The Poly-encoder \cite{Humeau2020Poly-encoders:} model generates multiple context-dependent representations of a document, thus providing a more nuanced view. These are then combined with the query through an attention mechanism, enhancing retrieval precision. The ColBERT \cite{khattab2020colbert} model goes a step further by creating dense vector representations for each individual token in the text. Its standout feature, termed      ``late interactions'', enables intricate interplay between individual query and text terms, a stark contrast to the standard cross-encoder design. 

% %The Poly-encoder model \cite{Humeau2020Poly-encoders:} addresses this by creating multiple context-dependent representations of a text, rather than one, offering varied views of the document. These representations are then aggregated via an attention mechanism with the query, facilitating nuanced interaction before final score computation, thereby enhancing retrieval accuracy and effectiveness.


% %The issue with bi-encoders is that the query and document are encoded independently, which means the model might fail to capture fine-grained, term-level interactions between them. The Poly-encoder \cite{Humeau2020Poly-encoders:} model was developed to address this limitation by generating multiple vector representations of a text from the corpus, rather than a single vector. This model learns multiple context codes, providing various perspectives of the corpus text, which are then aggregated into a single vector using an attention mechanism. The attention mechanism weighs the significance of each context code considering the query vector, enabling a nuanced interaction between the query and the various text representations before the final score computation. Even though the comparison function remains an inner product, similar to bi-encoders, the interaction with multiple representations allows the Poly-encoder model to offer improved accuracy and effectiveness in information retrieval. 

% %The ColBERT  \cite{khattab2020colbert} model takes this approach a step further by generating dense vector representations for each individual token in a given text. Their key innovation is a new comparison function that enables intricate interactions between individual query terms and the terms in the corpus text. This method, known as ``late interactions'', sharply contrasts with the all-to-all interactions observed in each transformer layer of the standard cross-encoder design. The ColBERT model showcases comparable effectiveness to cross-encoder designs but with significantly reduced query latency. 

% \textbf{Transformer Models.} Given BERT's over-parameterization, there is growing interest in exploring if smaller, task-specific models could achieve comparable success in NLP/IR tasks. One idea is to design new neural architectures from scratch to achieve better efficiency and effectiveness. This is evident in direct training of Transformers for document ranking tasks, with Hofstatter et al.'s Transformer Kernel \cite{hofstatter2019tu,hofstatter2020interpretable} (TK) model standing out for its separate transformer stacks that learn contextual representations of query and document terms. This model was later improved into the TK with local attention model \cite{hofstatter2020local} (TKL) that incorporated local self-attention. Further innovation was seen in Mitra et al.'s \cite{mitra2020conformer} Conformer Kernel (CK) model, an extension of TK, that added an explicit term-matching component and ``conformer'' layers.


% %BERT has been highly successful for various NLP/IR tasks, but given its over-parameterization, there is curiosity if smaller, task-specific models could be just as effective. One approach to this is through knowledge distillation, which transfers information from larger BERT models to smaller ones. However, this also raises the question of whether designing new neural architectures from the ground up could result in more optimal efficiency and effectiveness trade-offs. To study this, some researchers have directly trained Transformers for document ranking tasks. For example, Hofstatter et al.'s Transformer Kernel \cite{hofstatter2019tu,hofstatter2020interpretable} (TK) model learns contextual representations of query and document terms using separate transformer stacks. They further developed the TK model into the TK with local attention model (TKL) \cite{hofstatter2020local} that incorporates local self-attention. Mitra et al. \cite{mitra2020conformer} then expanded on TK, introducing the Conformer Kernel (CK) model that includes an explicit term-matching component and 'conformer' layers.

% \textbf{Seq2Seq Models.} 
% While tasks not resulting in a sequence of tokens were previously managed using encoder-only models like BERT, the advent of pre-trained sequence-to-sequence models such as T5 \cite{raffel2019exploring}, UniLM \cite{dong2019unified}, and BART  \cite{lewis2019bart} has spurred their application to a wider variety of NLP tasks. Building on this, Nogueira et al. \cite{nogueira2019document} proposed MonoT5, a model fine-tuned to estimate a document's relevance by assigning a probability to the ``true'' label during the initial decoding phase. The recent introduction of RankT5 \cite{zhuang2023rankt5} has further advanced this field, offering direct ranking scores for query-document pairs by fine-tuning the T5 model with pairwise or listwise ranking losses, significantly improving ranking performance and showcasing robust zero-shot ranking capabilities on out-of-domain data.



%Until recently, tasks that did not produce a sequence of tokens (e.g., document retrieval) were primarily addressed using encoder-only models like BERT. These models were well suited for classification tasks and token-level classification, taking advantage of BERT's \texttt{[CLS]} representation and \texttt{[SEP]} tokens. However, with the emergence of pre-trained sequence-to-sequence models such as T5 \cite{raffel2019exploring}, UniLM \cite{dong2019unified},  and BART \cite{lewis2019bart}, the exploration and application of these models for a variety of NLP tasks have increased. Building on the effectiveness of sequence-to-sequence models, Nogueira et al. \cite{nogueira2019document} proposed MonoT5 which uses a specific input format that incorporates a query and a document. The model is then fine-tuned to determine whether the document is relevant (``true'') or not relevant ("false") to the query. Similar to MonoBERT, MonoT5 is used as a reranking tool, and it estimates relevance by assigning a probability to the "true" label during the initial decoding phase. Recently, RankT5 \cite{zhuang2023rankt5} has been proposed which fine-tunes a T5 model with pairwise or listwise ranking losses. RankT5 is capable of generating direct ranking scores for query-document pairs, demonstrating significantly improved ranking performance across multiple public text ranking datasets, particularly exhibiting strong zero-shot ranking performance on out-of-domain data.




% \subsection{Neural Entity-Oriented Search}
% \label{subsec:Neural Entity-Oriented Search} 

%\textbf{Neural Entity-Oriented Search.} %Entity-oriented search  and neural-IR are two frontiers in IR that approach the field from different angles. The former leverages human knowledge and entity semantics from knowledge graphs, while the latter employs distributed representations and neural networks. 
%The Entity-Duet Ranking Model \cite{liu-etal-2018-entity} (EDRM) is a pioneering work that merges entity-oriented search and neural-IR paradigms. EDRM builds on the word-entity duet framework \cite{xiong2017word} and enhances it by harnessing the capabilities of neural networks and knowledge graphs. Recently, Tran and Yates \cite{tran2022dense} further developed this concept by proposing to cluster entities within documents to generate multiple ``views'' of the document. In contrast, in this work, we perceive entities within candidate documents as overarching concepts important for a comprehensive understanding of the query. We identify and prioritize entities (concepts) that align closely with the query. Different from prior work, we emphasize the embeddings of these important (relevant) entities and concurrently attenuate the less relevant ones within the document's representation, thus obtaining a refined, \textit{query-specific} document representation tailored for precise document ranking.

%to integrate BERT-based text representations with entity embeddings from the input text, generating multiple ``entity views'' that are then combined with the document's textual representation for efficient search.

%this concept was further developed by Tran and Yates \cite{tran2022dense}, who integrate BERT-based text representations with entity embeddings from the input text, generating multiple ``entity views'' that are then combined with the document's textual representation for efficient search.


%Entity-oriented search (Section \ref{subsec:Ad-hoc Document Retrieval Using Entities}) and dense retrieval (Section \ref{subsec:Dense Retrieval Using Transformers}) are frontiers of IR that push the boundaries from opposite ends. While entity-oriented search utilizes human knowledge and entity semantics from knowledge graphs, showing promising results in feature-based ranking systems, dense retrieval employs distributed representations and neural networks, facilitating the training of complex ranking models using vast datasets.

%The Entity-Duet Ranking Model \cite{liu-etal-2018-entity} (EDRM) is a pioneering work that examines whether the advantages of entity-oriented search in feature-based systems can be replicated in neural IR methodologies. This model blends the realms of neural search systems and entity-oriented search, creating an end-to-end learning architecture that combines both concepts smoothly. EDRM builds on the word-entity duet framework and enhances it by harnessing the capabilities of neural networks and the wealth of information from knowledge graphs.

%Despite EDRM's success, it wasn't until 2022 that Tran and Yates \cite{tran2022dense} revisited the use of knowledge graphs in neural search within the context of BERT. The crux of their approach lies in the amalgamation of a BERT-based text representation with an entity representation derived from entity embeddings in the input text. Instead of creating a single vector representation for all entities in a document, they produce multiple entity representations corresponding to different entity clusters in the text. These ``entity views'' are then combined with the document's textual representation and indexed for efficient search.

% \subsection{Retrieve-And-ReRank}
% \label{subsec:Retrieve-And-ReRank}

% The use of BERT for text ranking led to a significant 30\% improvement in performance on the MS MARCO passage ranking test collection, largely through a retrieve-and-rerank approach. This method, pioneered by Nogueira et al. in their model MonoBERT \cite{nogueira2019passage} and DuoBERT \cite{nogueira2019multi} models, treats the process as a relevance classification task. %This spurred exploration into multi-stage ranking \cite{nogueira2019multi}  architectures such as DuoBERT that balance effectiveness and efficiency by applying costlier features to candidates who pass initial relevance checks. 
% Furthermore, research has been dedicated to enhancing BERT's efficiency, with models such as 
% %DistilBERT \cite{sanh2019distilbert} reducing model size while retaining performance, and 
% RoBERTa \cite{liu2019roberta}, DeBERTa \cite{he2020deberta}, and ELECTRA \cite{clark2020electra} refining the pretraining and training processes to increase speed and effectiveness.


%BERT's application to text ranking revolutionized the field, showing a rapid 30\% improvement in effectiveness on the MS MARCO passage ranking test collection. This was achieved primarily through the retrieve-and-rerank approach, where BERT is applied to rerank initially retrieved texts. The pioneering implementation of this approach, called MonoBERT, was developed by Nogueira et al. \cite{nogueira2019passage} They designed MonoBERT as a relevance classification model, taking a query and a candidate text as input, producing a relevance score for the text with respect to the query.

%This groundbreaking work led to the exploration of multi-stage ranking architectures. The idea was to use cheaper features to discard obviously non-relevant candidates in the earlier stages and then apply more expensive features to the remaining candidates. This multi-stage design helps manage latency and offers system designers a balance between effectiveness and efficiency. Nogueira et al. again led the field by incorporating transformers into this multi-stage architecture in a model called DuoBERT \cite{nogueira2019multi}, which compared pairs of documents in a pairwise approach, leveraging comparisons between candidate texts to improve ranking.

%Following the success of BERT in IR/NLP tasks, there was a flurry of research into adapting the architecture to be more efficient and robust. For example, DistilBERT \cite{sanh2019distilbert} uses knowledge distillation during the pretraining phase to reduce the size of a BERT model by 40\%, retaining 97\% of its language understanding abilities, and making it 60\% faster. In a similar vein, RoBERTa \cite{liu2019roberta} removes the next-sentence pretraining objective, training with larger mini-batches, and increased learning rates. DeBERTa \cite{he2020deberta} builds on RoBERTa with disentangled attention and enhanced mask decoder training with half of the data used in RoBERTa. ELECTRA \cite{clark2020electra} trains two transformer models: the generator and the discriminator. The generator’s role is to replace tokens in a sequence, and is therefore trained as a masked language model. The discriminator tries to identify which tokens were replaced by the generator in the sequence.

% \subsection{Refining Query and Document Representations}
% \label{Refining Query and Document Representations}


\textbf{Query/Document Expansion.} %As we enrich the query and document representations using entity embeddings, our work is also related to work on query/document expansion and PRF. 
%One of the early works in query expansion using entities was by Dalton et al. \cite{dalton2014entity} who proposed the Entity-Query Feature Expansion (EQFE) model, harnessing explicit entity annotations within documents for query expansion. 
Recent efforts in this direction have been driven by embeddings. Solutions such as DeepCT \cite{dai2020context} and docT5query \cite{nogueira2019document} use transformers to enrich traditional PRF models by highlighting significant terms in documents. Simultaneously, methods like Neural PRF \cite{li-etal-2018-nprf} and BERT-QE \cite{zheng-etal-2020-bert} have adopted neural ranking models to measure document similarity with feedback documents. CEQE \cite{naseri2021ceqe} has further enhanced this approach by using BERT to create contextualized representations and select expansion terms based on similarity in the embedding space. While ColBERT-PRF \cite{xiao2023colbert-prf} directly utilizes BERT embeddings for retrieval without further training,  ANCE-PRF \cite{hongchien2021ance-prf} requires additional retraining of the query encoder using PRF information

%has distinguished itself by directly utilizing BERT embeddings for retrieval without further training, thereby circumventing potential topic drifts associated with polysemous words. In contrast, ANCE-PRF \cite{hongchien2021ance-prf}, which also employs BERT embeddings but requires additional retraining of the query encoder using PRF information. %Conversely, ColBERT-PRF operates effectively without the need for further training.



% Pseudo-relevance feedback (PRF) approaches have played a significant role in IR for many years, dating back to Rocchio's \cite{rocchio1971relevance} methods of refined query reformulations. Recently, deep learning solutions with transformer networks have been introduced, which expand on the statistical term information by rewriting or expanding the document collection. DeepCT \cite{dai2020context}, for instance, uses a fine-tuned BERT model to highlight important terms in documents, creating augmented document representations that can be traditionally indexed. In a similar vein, docT5query \cite{nogueira2019document} use text-to-text translation models to generate potential queries that could be relevant to a document, boosting retrieval effectiveness when these suggested queries are indexed with the original document. 

% There has also been a move towards using embeddings, instead of relying solely on statistical information. For example, Neural PRF \cite{li-etal-2018-nprf} and BERT-QE \cite{zheng-etal-2020-bert} are two methods that use neural ranking models to measure the similarity between a document and a top-ranked feedback document. Specifically, Neural PRF employs models like DRMM \cite{guo2016drmm} and KNRM \cite{xiong2017end}, while BERT-QE assesses similarity in relation to feedback chunks extracted from top-ranked feedback documents. CEQE \cite{naseri2021ceqe} selects expansion terms from top-ranked feedback documents that are closest to the query in the BERT embedding space. ColBERT-PRF \cite{xiao2023colbert-prf} uses BERT embeddings for retrieval, thus avoiding topic drifts for polysemous words. Unlike ANCE-PRF \cite{hongchien2021ance-prf}, which also aims to improve effectiveness by retraining the query encoder using pseudo-relevance feedback information, ColBERT-PRF doesn't require any further training.


% \subsection{Entity Ranking}
% \label{subsec:Entity Ranking}

\textbf{Entity Ranking.} %Entity ranking involves retrieving and ordering entities from a knowledge graph based on their relevance to a given query. 
%Earlier methods for entity ranking relied on term-based representations, using models like BM25 ~\cite{robertson2009probabilistic} to rank entities. 
Early methods include using MRFs to deal with the joint distribution of entity terms from semi-structured data ~\cite{metzler2005mrf,zhiltsov2015fielded,nikolaev2016paramterized,hasibi2016exploiting,raviv2012aranking}, utilizing types  ~\cite{kaptein2010entity,balog2011query,garigliotti2017on} and relations ~\cite{tonon2012combining,ciglan2012the} from a KG, and using Learning-To-Rank methods ~\cite{schuhmacher2015ranking,graus2016dynamic,dietz2019ent,chatterjee2021fine} to rank entities using a diverse set of features.
%
Recent advancements have been significantly driven by neural models using advanced techniques such as autoregressive entity ranking \cite{cao2021autoregressive}, integrating BERT-based entity rankings with other features \cite{chatterjee2022berter}, and enhancing BERT with Wikipedia2Vec \cite{yamada-etal-2020-wikipedia2vec} embeddings \cite{gerritse2022embert}.
%Models like GENRE \cite{cao2021autoregressive}, BERT-ER++ \cite{chatterjee2022berter}, and EM-BERT \cite{gerritse2022embert} have introduced advanced techniques such as autoregressive entity ranking, integrating BERT-based entity rankings with other features, and enhancing BERT with Wikipedia2Vec \cite{yamada-etal-2020-wikipedia2vec} embeddings. 
Concurrently, the emergence of graph embedding-based models ~\cite{gerritse2020graph,nikolaev2020joint} 
%such as GEEER ~\cite{gerritse2020graph} and KEWER ~\cite{nikolaev2020joint}, 
has enriched entity ranking approaches by utilizing joint embedding of entities and words within the same vector space. 
%Wikipedia2Vec \cite{yamada-etal-2020-wikipedia2vec} embeddings and enabling the joint embedding of entities and words within the same vector space.







% Given a query and a knowledge graph, the entity ranking task is to retrieve entities from this KG and order them by their relevance to the query. Traditional approaches create term-based representations or entity descriptions using unstructured sources or structured knowledge bases like DBpedia ~\cite{lehmann2015dbpedia}, which are then ranked using models like BM25 ~\cite{robertson2009probabilistic}. MRF-based models have been employed to deal with the joint distribution of entity terms from semi-structured data, as seen in the Sequential Dependence Model ~\cite{metzler2005mrf} and its variants \cite{zhiltsov2015fielded,nikolaev2016paramterized,hasibi2016exploiting,raviv2012aranking}. As large-scale KGs became available, semantically enriched models were developed that leverage entity types ~\cite{kaptein2010entity,balog2011query,garigliotti2017on} and relationships ~\cite{tonon2012combining,ciglan2012the} between entities.

% Recent strategies have pivoted towards Learning-To-Rank (LTR) methods ~\cite{schuhmacher2015ranking,graus2016dynamic,dietz2019ent,chatterjee2021fine}, which use diverse features to re-rank entities, with textual information and neighboring relationships becoming focal points. The introduction of graph embedding-based models, such as GEEER ~\cite{gerritse2020graph} and KEWER ~\cite{nikolaev2020joint}, has also added a new dimension to entity ranking by leveraging Wikipedia2Vec \cite{yamada-etal-2020-wikipedia2vec}  embeddings and jointly embedding entities and words in the same vector space.

% The latest advancements in the field have been driven by transformer-based neural models like GENRE \cite{cao2021autoregressive}, BERT-ER++ \cite{chatterjee2022berter}, and EM-BERT  \cite{gerritse2022embert}. These models offer advanced techniques such as autoregressive entity ranking, blending BERT-based entity rankings with other features, and augmenting BERT with Wikipedia2Vec entities, effectively revolutionizing entity ranking methods and their performance.

% \subsection{Knowledge-Enhanced BERT}
% \label{subsec:Knowledge-Enhanced BERT}
% Recently, there has been much research on learning entity-enriched BERT models. ERNIE \cite{zhang-etal-2019-ernie} uses vectors from TransE \cite{bordes2013transe} whereas KnowBert ~\cite{peters-etal-2019-knowledge} uses a word-to-entity attention to integrate knowledge about entities into BERT.  E-BERT ~\cite{poerner-et-al-2020-ebert} aligns entity vectors from Wikipedia2Vec ~\cite{yamada-etal-2020-wikipedia2vec}  with BERT's vectors and outperforms both ERNIE and KnowBert on several NLP tasks. KEPLER ~\cite{wang-etal-2021-kepler} aligns the semantic space of text to the symbolic space of knowledge graphs by using entity descriptions as a bridge and jointly optimizing the knowledge embedding and the masked language modeling objectives. %K-ADAPTER \cite{wang-etal-2021-k} injects (1) factual knowledge obtained from Wikipedia. and (2) linguistic knowledge obtained via dependency parsing using a neural adapter for each kind of infused knowledge with no information flow between different adapters. 
 
% \subsection{Graph Embeddings}
% \label{subsec:Entity Embeddings}

% There is extensive research on learning entity embeddings through knowledge graphs. TransE ~\cite{bordes2013transe} is a prominent method that represents relationships between entities as translations between their embeddings. Variations such as TransH ~\cite{wang2014transh} and TransR ~\cite{lin2015transr} represent relations with distinct vectors or in different spaces, respectively. DistMult  ~\cite{yang2014embedding} combines these two entity vectors via a relation-specific function, while SimplE ~\cite{kazemi2018simple} employs tensor factorization to learn separate entity embeddings for head and tail roles. Models like ComplEx ~\cite{trouillon2016complex} and RotatE \cite{sun2019rotate} project entities to the complex vector space and use dot products or rotations for relation learning. QuatE ~\cite{zhang2019quate} takes it a step further by using hypercomplex-valued embeddings in quaternion space. Wikipedia2Vec ~\cite{yamada-etal-2020-wikipedia2vec} uses the skip-gram model ~\cite{Mikolov2013Distributed} to learn entity embeddings.

% There has been much work on learning entity embeddings using knowledge graphs. %We provide a brief overview of some below. 
% %
% TransE ~\cite{bordes2013transe} learns embeddings for both entities and relations based on the idea that the relationship between two entities corresponds to a translation between the embedding of these entities. 
% Several variations of the TransE model have been proposed. For example, 
% TransH ~\cite{wang2014transh} represents each relation with two vectors: a norm vector and a translation vector whereas TransR ~\cite{lin2015transr} models entities and relations in a distinct entity space and multiple relation spaces. DistMult ~\cite{yang2014embedding} projects an entity pair to low dimensional vector space, then combines these two vectors via a scoring function with relation-specific parameters. SimplE ~\cite{kazemi2018simple} is a tensor factorization approach %based on canonical Polyadic decomposition \cite{hitchcock1927expression} 
% that learns one embedding vector for each relation and two embedding vectors for each entity, one to be used when the entity is the head and one to be used when the entity is the tail. To capture anti-symmetric relations between entities, ComplEx ~\cite{trouillon2016complex} projects entities to the complex vector space and learns embedding using the dot product. Similarly, RotatE \cite{sun2019rotate} maps the entities and relations to the complex vector space and defines each relation as a rotation from the source entity to the target entity. QuatE ~\cite{zhang2019quate} uses hypercomplex-valued embeddings with three imaginary components to represent entities. Relations are modelled as rotations in the quaternion space. Wikipedia2Vec ~\cite{yamada-etal-2020-wikipedia2vec} uses the skip-gram model ~\cite{Mikolov2013Distributed} to learn entity embeddings.



==> tex-files/subsections/research-questions.tex <==
\subsection{Research Questions}
\label{subsec:Research Questions}

As we use \texttt{DREQ} to re-rank a candidate set of documents, the first question we ask is: \textbf{(RQ1)} \textit{How does \texttt{DREQ} perform in comparison to state-of-the-art document re-ranking methods? Which type of queries does it help the most?} 
%As our work aims to improve precision of the re-ranked candidate set, we ask: \textbf{(RQ2)} \textit{How effective is \texttt{DREQ} in improving the precision at top ranks of the reranked results? To what extent do entities contribute to this?}
Entities lie at the heart of our approach. Hence, we ask: \textbf{(RQ2)} \textit{What is the contribution of entities in \texttt{DREQ}? How does the performance change if we change the underlying entity ranking system?} Furthermore, \textbf{(RQ3)} \textit{How does changing the entity weighing method alter the performance of \texttt{DREQ}?}
%To complete the analysis, we ask: \textbf{(RQ3)} \textit{How does \texttt{DREQ} perform when compared to SOTA full retrieval methods?} 
%As our work is related to neural query and document expansion, we compare our work to several neural PRF methods, in addition to other SOTA full retrieval methods.
%We address the following research questions in this work.

% \begin{enumerate}[leftmargin=*]


%     \item[\textbf{RQ1}] How does DREQ perform in comparison to state-of-the-art neural and non-neural re-rankers? Which type of queries does it help the most? 
    
%     \item[\textbf{RQ2}] What is the reason for the superior performance of DREQ? To what extent do entities contribute to this improvement?
    
%     \item[\textbf{RQ3}] What role does entity ranking play in DREQ? How does the performance of DREQ change if we change the underlying entity ranking system?
    
%     %\item[\textbf{RQ4}] What is the effect of weighing the entity embeddings using the entity scores? How does the performance change if we do not weigh the embeddings?

%     \item[\textbf{RQ4}] How does the performance of DREQ vary when varying the number of top-$k$ entities chosen from the entity ranking?

%     \item[\textbf{RQ5}] How does DREQ perform in comparison to SOTA full retrieval methods? 
% \end{enumerate}

==> tex-files/subsections/results-alternative-entity-weights.tex <==
\subsection{Alternative Entity Weighing in \texttt{DREQ}}
\label{subsec:Alternative Entity Weighing}
 
The \texttt{DREQ} model intrinsically uses entity scores, expressed as probabilities, to weight the entity embeddings within documents. Acknowledging the pivotal role these probabilistic weightings have in shaping the model's performance, we perform a series of experiments to examine various alternative weighting schemes. In the following, \textbf{we discuss results with respect to only Robust04 (title)}.

\textbf{Uniform Weights.} First, we remove entity weightings, treating all entities with equivalent importance within the document's representation. This leads to a significant performance decrease in \texttt{DREQ}, from an nDCG@20 of 0.75 to 0.70. The difficulty test, using the BM25+RM3 candidate ranking, shows that \texttt{DREQ} using uniform weights helps 187 queries, whereas the original model helps 210. 

% As an additional experiment, we weigh the entity embeddings using the reciprocal rank of the entities from the entity ranking instead of their rank scores. Again, we observe a significant performance decrease in \texttt{DREQ}, from an nDCG@20 of 0.75 to 0.54.

%This downturn further underscores the pivotal role of entities in \texttt{DREQ}; appropriately weighted embeddings amplify the semantic alignment between queries and documents, attesting to our intuition earlier. Moreover, the drop in performance indicates the foundational role of the entity ranking mechanism in \texttt{DREQ}. 

%It's clear that the ranking system's ability to discern and prioritize query-relevant entities is instrumental to the success of \texttt{DREQ}. %It's crucial to assess the relevance of entities to the query, not just identify them.
%
%To further dissect the influence of the entity ranking system, we removed entity weightings (treating all entities with equivalent importance within the document's representation), thereby rendering the ranker's output moot. We find that this leads to a significant decrease in performance of \texttt{DREQ}, from an nDCG@20 of 0.75 (using rank scores as weights) to 0.70. Performing the difficulty test described above using the BM25+RM3 candidate ranking, we find that \texttt{DREQ} using uniform entity weights helps 187 queries; in contrast, the full \texttt{DREQ} model helps 210.

This downturn underscores the pivotal role of entities in \texttt{DREQ}. Their embeddings, when appropriately weighted by relevance probabilities, significantly amplify the semantic alignment between queries and documents, attesting to the strategic decision to utilize them. Their importance becomes glaringly evident when their individual significance is disregarded, leading to a diluted representation that hampers the model's performance. Furthermore, it's clear that the ranking system's role isn't merely ornamental; its ability to discern and prioritize entity relevance is instrumental to \texttt{DREQ}'s success. Beyond just pinpointing entities, the ability to gauge their importance vis-à-vis the query is paramount.

%However, this experiment doesn't just elucidate the value of entities; it also shines a light on the significance of the entity ranking system. By nullifying the weights, we effectively rendered the output of the ranking system moot, leading to a neutral representation. The aforementioned drop in performance, in this context, indicates the foundational role of the entity ranking mechanism in DREQ. It's clear that the ranking system's role isn't merely ornamental; its ability to discern and prioritize entity relevance is instrumental to \texttt{DREQ}'s success. Beyond just pinpointing entities, the ability to gauge their relevance vis-à-vis the query is paramount.

\textbf{Reciprocal Rank.} Additionally, we explore the reciprocal rank (RR) of entities as an alternative weighting mechanism for entity embeddings. The results are telling: nDCG@20 plummets from 0.75 to 0.54. The RR method assumes a precipitous decrease in the importance of entities based on rank. However, this isn't always fitting. Take for instance the query ``Black Bear Attacks''. The entity \textit{George Parks Highway}, with a score of 0.99, is ranked 71st, while \textit{Cantwell, Alaska}, with a nearly identical score of 0.98, stands at 106th rank. Such negligible probability differences juxtaposed against substantial rank disparities highlight the potential limitations of the RR system. It underscores the risk of undervaluing entities that, by probability, are nearly as pertinent as top-tier entities.

\textbf{\textit{Take-Away.}} In addressing \textbf{(RQ3)}, our experiments unveil crucial insights. The inherent design of \texttt{DREQ}, which uses entity scores as probabilities to weight the entity embeddings, stands out as a potent approach, demonstrated by superior performance metrics. When entities are uniformly weighted, stripping them of their probabilistic distinctions, the model's performance takes a tangible hit, underscoring the model's dependence on the nuanced gradation of entity relevance. The experiment with RR as weights further cements this observation. While RR attempts to rank entities based on their ordinal positions, it fails to adequately capture the subtleties in actual relevance, particularly when entities with near-identical probabilities have significantly differing ranks. The experiments not only re-emphasize the instrumental role of entities in \texttt{DREQ} (\textbf{RQ2)}, but also the imperativeness of a precise entity ranking and weighting mechanism.

%In conclusion, this comparison not only re-emphasizes the instrumental role of entities in \texttt{DREQ} (\textbf{RQ2)}, but also the imperativeness of a precise entity ranking and weighting mechanism. The effectiveness of \texttt{DREQ} is keenly influenced by how entities are weighed — particularly when these weights are distilled from normalized probability scores. The comparative analysis underlines the importance of gauging entities' relative significance to the query with precision.

%The RR method presumes a sharp decline in the significance of entities as they are ranked lower. This presupposition, however, doesn't necessarily resonate with all scenarios. Often, top-ranked entities can bear nearly equivalent relevance to the query. In such instances, the reciprocal rank's approach to sharply reducing weights for marginally lower-ranked entities proves detrimental.

%As an additional experiment, we weigh the entity embeddings using the reciprocal rank of the entities from the entity ranking instead of their rank scores. Again, we observe a significant performance decrease in \texttt{DREQ}, from an nDCG@20 of 0.75 to 0.54. The reciprocal rank assumes that the importance of entities decreases rapidly as one moves down the rank. This assumption might not always hold true. There might be several top-ranked entities that are almost equally relevant to the query. In such cases, assigning drastically reduced weights to slightly lower-ranked entities might be counterproductive. Examining the entity ranking for the query ``Black Bear Attacks'', we observe that the entity \textit{George Parks Highway} receives a rank score of 0.99 and placed at rank 71 whereas the 




==> tex-files/subsections/results-dreq-vs-full-ret.tex <==
\subsection{Comparison to Full Retrieval}
\label{subsec:Comparison to Full Retrieval}

\input{tex-files/tables/results-full-ret}

While \texttt{DREQ} is primarily a re-ranking method, we also benchmark it against full retrieval methods for a thorough performance evaluation. \textbf{Results on only Robust04 (title) are shown} in Table \ref{tab:res-tab-full-ret} due to space limitations.
%While \texttt{DREQ} is fundamentally a re-ranking method, we also compare its performance with full retrieval methods to provides a comprehensive performance benchmark. Results on only Robust04 (title) are shown in Table \ref{tab:res-tab-full-ret} due to space constraints.
%as full retrieval methods represent the current state-of-the-art and are widely used in practice. We choose a wide array of state-of-the-art full retrieval methods (see Section \ref{subsec:Baselines}).
%Due to space constraints, we only show results on Robust04 (title) in Table \ref{tab:res-tab-full-ret}. 

We observe that \texttt{DREQ} consistently surpasses the performance of all baseline full retrieval methods. To illustrate, the highest performing full retrieval method, BERT-QE, achieves a $\text{MAP}=0.39$ and $\text{nDCG@20}=0.55$. Impressively, our model, \texttt{DREQ}, enhances this by 44\% in terms of MAP and 36\% in terms of nDCG@20. A more granular analysis reveals that \texttt{DREQ} improves performance for 182 out of the 250 queries where BERT-QE struggles. When we apply the difficulty test delineated in Section \ref{subsec:Contribution of Entities} utilizing the WIG method, it becomes evident that \texttt{DREQ} not only elevates the performance for easy queries but also significantly for the most challenging ones.
%
The remarkable performance of \texttt{DREQ} across a spectrum of query difficulties, including the most challenging ones, underscores its robustness and superiority over existing full retrieval methods. %This highlights the pivotal role of \texttt{DREQ} in enhancing the efficacy of document retrieval and relevance interpretation, thereby paving the way for more accurate and efficient information retrieval systems.

%We observe that \texttt{DREQ} outperforms all baseline full retrieval methods. For example, the best performing full retrival method BERT-QE achieves $\text{MAP}=0.39$ and $\text{nDCG@20}=0.55$. Our model \textit{DREQ} improves upon this by 44\% in terms of MAP and 36\% in terms of nDCG@20. On further analysis, we find that \texttt{DREQ} improves performance for 182 of the 250 queries for which BERT-QE does not perform well. Performing the difficulty test described in Section \ref{subsec:Contribution of Entities} using the WIG method, we find that \texttt{DREQ} not only improves performance of the easy queries but also of the most difficult ones.

\textbf{\textit{Take Away.}} To answer \textbf{RQ3}, \texttt{DREQ} outperforms several state-of-the-art full retrieval methods. While \texttt{DREQ} is a re-ranking system, its ability to outperform full retrieval models, even when starting with a simple candidate set, suggests that incorporating entities in the retrieval process holds significant potential. %This not only underscores the efficacy of \texttt{DREQ} and the entity-centric approach it employs but also opens up avenues for further exploration and optimization in information retrieval, with a particular focus on leveraging entities



==> tex-files/tables/results-ablation-study.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Ablation study results on \textbf{TREC Robust 2004 title queries}. Only best reranking baselines shown. $\blacktriangleup$ denotes significant improvement and $\blacktriangledown$ denotes significant deterioration compared $\star$ using a paired-t-test at $p<0.05$.}
\label{tab:res-tab-ablation-study}
\begin{tabularx}{\textwidth}{|l|CCC|}
\hline
            & \textbf{MAP@20}  & \textbf{nDCG@20} & \textbf{P@20} \\ \hline
BM25+RM3    & 0.16     & 0.44        & 0.37     \\ \hline 
RankT5  & 0.17           & 0.50            & 0.43      \\ 
ConvBERT       & 0.18           & 0.52           & 0.45       \\
CEDR     & 0.20           & 0.55           & 0.48 \\ \hline
%DREQ (No Query Entity Embedding)        & -- & --    & -- \\ \hline
%DREQ (No Document Entity Embedding)        & -- & --    & -- \\ \hline
DREQ (Only Text Embedding)        & 0.06 & 0.26    & 0.23 \\ \hline
DREQ (Full)        & 0.37 & 0.75    & 0.73 \\ \hline
\end{tabularx}
\end{table}

==> tex-files/tables/results-change-entity-ranking.tex <==

\begin{table}[t]
\centering
\caption{Results on \textbf{TREC Robust 2004 title queries} for replacing our BERT-based entity ranking with entity rankings obtained using other methods. $\blacktriangleup$ denotes significant improvement and $\blacktriangledown$ denotes significant deterioration compared to \textit{BERT} (denoted $\star$) using a paired-t-test at $p<0.05$.}
\label{tab:res-tab-change-entity-ranking}
\begin{tabularx}{\textwidth}{|l|CC|CC|}
\hline
                      & \multicolumn{2}{c|}{\textbf{Entity Ranking}} & \multicolumn{2}{c|}{\textbf{Document Ranking}} \\ \hline
Entity Ranking Method & \textbf{MAP}              & \textbf{P@20}             & \textbf{MAP}              & \textbf{nDCG@20}            \\ \hline
\textbf{BERT}                  & $\mathbf{0.94}$             &  $\mathbf{0.97}$             &  $\mathbf{0.56}$             &  $\mathbf{0.75}$  \\ \hline 
BM25+RM3              & 0.27             & 0.57             & 0.27             & 0.44               \\
GEEER                 & 0.29             & 0.63             & 0.25             & 0.42               \\
\hline
\end{tabularx}
\end{table}


==> tex-files/tables/results-change-entity-weighing-method.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Results on \textbf{TREC Robust 2004 title queries} comparing different entity weighing methods in DREQ. Only best reranking baselines shown. $\blacktriangleup$ denotes significant improvement and $\blacktriangledown$ denotes significant deterioration compared to BM25+RM3 (denoted $\star$) using a paired-t-test at $p<0.05$.}
\label{tab:res-tab-change-entity-weighing-method}
\begin{tabularx}{\textwidth}{|l|CCC|}
\hline
            & \textbf{MAP@20}  & \textbf{nDCG@20} & \textbf{P@20} \\ \hline
BM25+RM3    & 0.16           & 0.44           & 0.38        \\ \hline
RankT5  & 0.17           & 0.50            & 0.43      \\ 
ConvBERT       & 0.18           & 0.52           & 0.45       \\
CEDR     & 0.20           & 0.55           & 0.48 \\ \hline
DREQ (Uniform)  & 0.32 & 0.70 & 0.66 \\ \hline
DREQ (Inverse Log Rank)  & 0.33 & 0.71 & 0.68 \\ \hline
DREQ (Reciprocal Rank)  & 0.24 & 0.54 & 0.48 \\ \hline
DREQ (RetScore)    & 0.37 & 0.75    & 0.73 \\ \hline
\end{tabularx}
\end{table}

==> tex-files/tables/results-full-ret.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t]
\centering
\caption{Results on \textbf{TREC Robust 2004 title queries} comparing DREQ to full retrieval methods. 
%Top: Query/document expansion full retrieval methods. Bottom: Full retrieval methods not using query/document expansion. 
\textbf{Note: DREQ is reranking the BM25+RM3 full retrieval results presented at the top.} $\blacktriangle$ denotes significant improvement and $\blacktriangledown$ denotes significant deterioration compared to BM25+RM3 (denoted $\star$) using a paired-t-test at $p<0.05$.}
\label{tab:res-tab-full-ret}
\scalebox{0.8}{
\begin{tabularx}{\textwidth}{|l|CCCC|}
\hline
            & \textbf{MAP}  & \textbf{nDCG@20} & \textbf{P@20} & \textbf{MRR} %&\textbf{R@1000}
            \\ \hline
BM25+RM3    & 0.29     & 0.44        & 0.38 & 0.37 %& 0.78   
\\ \hline 
BERT-QE     & 0.39 & 0.55    & 0.49 & 0.78 %& 0.78
\\
CEQE     & 0.31 & 0.46    & 0.40 &  0.68 %& 0.78
\\
DeepCT      & 0.20  & 0.38    & 0.33 & 0.63 %& 0.59
\\
NPRF        & 0.29 & 0.45    & 0.41 & --\\
EQFE        & 0.33 & 0.43    & 0.38 & 0.65 %& 0.81
\\ %\hline
ANCE     & 0.13 & 0.31 & 0.25   & 0.61 %& 0.48 
\\
BERT-MaxP      & 0.31  & 0.48 & 0.42   & 0.73 %&0.78 
\\
TCT-ColBERT        & 0.23 & 0.43 & 0.36   & 0.74 %& 0.64
\\
PARADE        & 0.30 & 0.52 & 0.45   & 0.81 %& 0.70
\\
SPLADE        & 0.22 & 0.42 & 0.36   & 0.68 %& 0.60
\\ \hline
\textbf{DREQ}        & $\mathbf{0.56}$ & $\mathbf{0.75}$    & $\mathbf{0.73}$ & $\mathbf{0.97}$ %& 0.68
\\ \hline
\end{tabularx}
}
\end{table}
